Automated Tiling of Unstructured Mesh Computations with Application to Seismological Modelling

Sparse tiling is a technique to fuse loops that access common data, thus increasing data locality. Unlike traditional loop fusion or blocking, the loops may have different iteration spaces and access shared datasets through indirect memory accesses, such as A[map[i]] -- hence the name "sparse". One notable example of such loops arises in discontinuous-Galerkin finite element methods, because of the computation of numerical integrals over different domains (e.g., cells, facets). The major challenge with sparse tiling is implementation -- not only is it cumbersome to understand and synthesize, but it is also onerous to maintain and generalize, as it requires a complete rewrite of the bulk of the numerical computation. In this article, we propose an approach to extend the applicability of sparse tiling based on raising the level of abstraction. Through a sequence of compiler passes, the mathematical specification of a problem is progressively lowered, and eventually sparse-tiled C for-loops are generated. Besides automation, we advance the state-of-the-art by introducing: a revisited, more efficient sparse tiling algorithm; support for distributed-memory parallelism; a range of fine-grained optimizations for increased run-time performance; implementation in a publicly-available library, SLOPE; and an in-depth study of the performance impact in Seigen, a real-world elastic wave equation solver for seismological problems, which shows speed-ups up to 1.28x on a platform consisting of 896 Intel Broadwell cores.

==> Makefile <==
PACKAGE=acmart

SAMPLES=seigen-tiling.tex

PDF = ${SAMPLES:%.tex=%.pdf}

all:  clean ${PDF}
	rm -f comment.cut

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

seigen-tiling.pdf: body.tex

diff.pdf: cleandiff diff.tex

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

cleandiff:
	rm -f diff.{aux,log,out,bbl,blg}

clean:
	@$(RM) seigen-tiling.pdf *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

gendiff:
	latexdiff --flatten original/seigen-tiling.tex seigen-tiling.tex > diff.tex

gendiff-rebuttal1:
	latexdiff --flatten rebuttal_1/seigen-tiling.tex seigen-tiling.tex > diff.tex

diff: gendiff diff.pdf

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

